Robust Remote Reinforcement Learning over Unreliable Communication Channels using Homomorphic State Encoding

Traditional Reinforcement Learning (RL) frameworks generally assume that the agent perceives the state of the underlying Markov process instantaneously and then takes actions accordingly. If the agent cannot directly observe the process, but rather receives state updates from a remote sensor over a lossy and/or delayed channel, it may be forced to operate with partial and intermittent information. In recent years, numerous learning architectures have been proposed to manage RL with imperfect or remote feedback; however, they offer solutions tailored to specific use cases, often with a substantial computational and communication burden. To address these limitations, we propose a novel learning architecture, named Homomorphic Robust Remote Reinforcement Learning (HR3L), that enables the distributed training of RL agents over unreliable communication channels without the need to exchange gradient information. Our experimental results demonstrate that HR3L significantly outperforms the state-of-the-art methods in terms of sample efficiency, leading to faster training and reduced communication overhead. In addition, we show that HR3L can adapt to different scenarios, including packet loss, delayed transmissions, and bandwidth limitations, without experiencing significant performance degradation.

==> info_bottleneck.tex <==


\subsection{Theoretical Interpretation}

In our system, the characteristics of the channel constrain the receiver's ability to perceive the state of the environment.
Importantly, the receiver is allowed to use all previous messages to compute an \emph{a priori} belief distribution of the next state $s_{t+1} \in \mathcal{S}$.
To this end, the receiver can take advantage of the transition probability function $P$ of Def.~\ref{def:rrl}, which can be known in advance or learned. 
Therefore, the transmitter only needs to communicate the information that the receiver is unable to autonomously predict.

Given all received messages $\hat m_{1:t}$ up to the current slot $t$, the joint optimization of the encoding and control strategies can be written as
\begin{equation}
\label{eq:rmdp}
\begin{split}
    &\max_{\lambda, \pi} \mathbb{E}_{a_t \sim \pi(p_{\hat s_t})} [G(t)] \\ 
    &\mathrm{s.t.} \ I(s_t, \hat m_t \mid \hat m_{1:t-1}) \leq C \,,
\end{split}
\end{equation}
where $I(s_t, m_t \mid m_{1:t-1})$ is the conditional mutual information between $s_t$ and $\hat m_t$ given all past messages, defined as
% In the above equation, $I(s_t, m_t \mid m_{1:t-1})$ is the conditional mutual information between $s_t$ and $m_t$ given all past messages, and represents the additional information about the state $s_t$ carried by the last message $m_t$ and is not present in $m_{1:t-1}$.
% The value of $I(s_t, m_t \mid m_{1:t-1})$ is obtained as
\begin{equation}
    I(s_t,\hat m_t \mid \hat m_{1:t-1}) = I(s_t,\hat m_{1:t}) - I(s_t, \hat m_{1:t-1}).
\end{equation}
In the above equation, $I(s_t, \hat m_{1:t-1})$ is the information that the receiver can infer about state $s_t$ before receiving message $\hat m_t$, while $I(s_t,\hat m_{1:t})$ is the mutual information between state $s_t$ and the entire sequence of messages $\hat m_{1:t}$.
Therefore, $I(s_t, m_t \mid m_{1:t-1})$ represents the additional information about the state $s_t$ carried by the last message $\hat m_t$, which cannot exceed the channel capacity $C$
%This denotes how messages incrementally help reconstruct the state

This formulation clarifies the importance of designing a transmitter that keeps track of not only the current state of the environment $s_t$, but also of the information available to the receiver.
On the other hand, the receiver must maintain a history of past messages $m_{1:t}$, or a belief $p_{\hat s_t}$ that is statistically equivalent to it, to limit redundancy between subsequent transmissions.


==> prev_model.tex <==

\begin{figure}[tbhp]
   \centering
   \include{schemes/system_model}
   \caption{Reference Remote Markov Decision Process (RMDP) scheme.}
   \label{fig:system_model}
\end{figure}

\section{System Model}
\label{sec:model}
We consider a \acrfull{rrl} push-based model with two agents, namely the \emph{transmitter} (or observer) and the \emph{receiver} (or controller), as shown in Fig.~\ref{fig:system_model}.
The transmitter observes the state of a certain process (that is, the \textit{environment)} and sends a compressed version of its observations to the receiver, which controls the system to maximize a reward signal. Contrary to most state-of-the-art models, we consider a non-ideal communication channel, with capacity limits, delays, and packet losses.

According to the push-based paradigm, communication and control policies jointly determine the system's performance. 
The transmitter must learn how to encode the  observations according to a \gls{goc} approach, to help the receiver make its control decisions. In turn, the receiver must learn to choose control actions based on the information received through the communication channel. 
Intuitively, both communication and control policies must account for channel conditions.

The system model is mathematically formalized as follows.
\subsection{Remote Markov Decision Processes}
\label{subsec:rmdp}
Let $\Delta(\Omega)$ indicate the set of all probability distributions with support in the discrete set $\Omega$.

We assume that the time is discretized in steps $t=0,1,2,\ldots$, and we model the target system as an infinite-horizon \gls{rmdp}, as defined below. 
\begin{definition}
\label{def:rrl}
An infinite-horizon \gls{rmdp} is a tuple $\langle \mc{S}, \mc{A}, \mc{M}, \mc{C}, P, r, \gamma \rangle$, where:
  \begin{itemize}
    \item $\mc{S}$ is the set of possible states;
    \item $\mc{A}$ is the set of possible actions;
    \item $\mc{M}$ is the set of possible messages;
    \item $\mc{C}$ is the communication channel model;
    \item $P:\mc{S}\times\mc{A} \times\mc{S}
    \to [0,1]$ is the state transition probability function;
    \item $r:\mc{S}\times\mc{A}\to\mathbb{R}$ is the reward function;
    \item $\gamma \in [0,1)$ is the exponential discount factor.
  \end{itemize}
\end{definition}
The state transition matrix $P$ describes the statistical evolution of the system in time: given the current state $s_t$ and the control action $a_t \in \mc{A}$, the system moves to state $s_{t+1} \in \mc{S}$ with probability $P(s_t, a_t, s_{t+1})$. 
However, in \gls{rrl} the receiver generally does not have perfect knowledge of the current state of the system $s_t$, but rather maintains a \emph{belief} $p_{\hat s_t}\in \Delta(\mc{S})$ of the current state, based on the messages $\hat m_{1:t}$ received up to time $t$ through the channel $\mc{C}$, and takes control decision based on this belief.
%At each time step $t$, the receiver takes an action $a_t \in \mc{A}$ and the system evolves from state $s_t$ to state $s_{t+1} \in \mc{S}$ with probability $P(s_t, a_t, s_{t+1})$.
%The receiver must learn a control policy $\pi:\Delta(\mc{S})\to\Delta(\mc{A})$ that maps the receiver's \emph{beliefs} over the system's state to action probabilities.
%As in traditional \glspl{mdp}, 
The final goal of the control policy is to maximize the long-term reward, which in our case is accessible only to the receiver.\footnote{We observe that this restriction, which is realistic in remote control scenarios, is mostly neglected in the literature on \gls{rrl}, where the reward is assumed to be immediately available to all agents~\cite{tung2021effective}.
} Therefore, the optimal control policy $\pi^*$ maps the current belief $p_{\hat s_t}$ into a probability distribution over the action space to maximize the expected long-term discounted reward:
\begin{equation}
\label{eq:optimal_control}
    \pi^* = \argmax_{\pi:\Delta(\mc{S})\to\Delta(\mc{A})} \mathbb{E}_{a_t \sim \pi(p_{\hat s_t})} \left[ G(t) \right],
\end{equation}
where $G(t)=\sum_{t=0}^\infty \gamma^t r(s_t,a_t)$, and the expectation is taken over the probability distribution of the action given by $\pi$. 


%Note that the control policy does not operate directly in the state space, but in the \textit{belief} space $\Delta(\mc{S})$.

On the sender side, the transmitter observes the system's state $s_t \in \mc{S}$  at each time step $t$, and encodes it in a message $m_t =\lambda(s_t) \in \mc{M}$ through an encoding function $\lambda:\mc{S}\to\mc{M}$. Note that, in general, the encoding process can be lossy, so the state $s_t$ may not be fully recoverable from $m_t$. The challenge for the transmitter is to learn an encoding policy $\lambda$ that helps the receiver maximize the expectation of $G(t)$, despite channel impairments.  
%The transmitter's goal is the same as the receiver's: therefore, the optimal encoding policy $\lambda^*$ is the one that maximizes the expectation of $G(t)$, which also depends on the receiver's control policy $\pi$.
The transmitter then affects the reward indirectly through its effect on the receiver's beliefs over the system state. 

\subsection{Communication Channel}
\label{subsec:cc}
As mentioned, the non-idealities of the transmission channel impact the encoding and control policies. In this study, we consider a channel model with the following characteristics:\\
%Capacity, delay, and packet loss.
- \textit{capacity} ($C$): it determines the maximum length $L$ of the message that can be transmitted in a time slot;\\
- \textit{delay}: it determines the number $d_t$ of time steps after which the receiver gets the message $m_t$ sent at time $t$.
In this work, we first consider $d_t$ to be constant, and then we address a scenario with stochastic delays. 
- \textit{packet loss}: we consider a markovian Gilbert-Elliot erasure channel model, where packets are successfully delivered if the channel is in Good state, and erased with probability $p>0$ in the Bad state. The transition probabilities between the two states determine not only the average probability of erasure but also the average duration of good and bad periods, making it possible to investigate the robustness of \gls{rrl} strategies to bursts of packet losses. This model advances the existing literature, where packet erasures are typically assumed to follow a Bernoulli process with stationary loss probability $p$~\cite{chen2024efficient}. 

Finally, we assume that the reward signal $r_t$ is available only to the receiver, which can share it asynchronously with the transmitter~\cite{tung2021effective}, before the end of each training round.
Being asynchronous, the return channel is not critical, since packets can be retransmitted until sucess, without any consequence for the training process.

\subsection{Theoretical Interpretation}

In our scenario, the characteristics of the channel constrain the capability of the receiver to observe the system's state.
% For a given channel capacity $C$, the information available to a \textit{memoryless} receiver regarding the system state is bounded by
% \begin{equation}
% \label{eq:information}
% I(s_t,m_t) \leq C\,,
% \end{equation}
% where $I(s_t,m_t)$ denotes the mutual information between the state $s_t$ and the received message $m_t$. 
% This bound holds when each observation $s_t$ is encoded and decoded independently, in accordance with the memoryless property.
%However, in our scenario, the observations are time correlated and the receiver can exploit this correlation to enhance its accuracy in estimating the current state. 
%In practice, 
In our scenario, 
the receiver can use the previous messages to compute an \emph{a priori} belief distribution over the next state, taking advantage of the transition probability function $P$ from Def.~\ref{def:rrl}, which can be known in advance or learned. 
In this case, the transmitter only needs to communicate the information that the receiver is unable to autonomously predict.

Given all received messages $\hat m_{1:t}$ up to the current time step $t$, the joint optimization of the encoding and control strategies can be written as
\begin{equation}
\label{eq:rmdp}
\begin{split}
    &\max_{\lambda, \pi} \mathbb{E}_{a_t \sim \pi(p_{\hat s_t})} [G(t)] \\ 
    &\mathrm{s.t.} \ I(s_t, \hat m_t \mid \hat m_{1:t-1}) \leq C \,,
\end{split}
\end{equation}
with 

% In the above equation, $I(s_t, m_t \mid m_{1:t-1})$ is the conditional mutual information between $s_t$ and $m_t$ given all past messages, and represents the additional information about the state $s_t$ carried by the last message $m_t$ and is not present in $m_{1:t-1}$.
% The value of $I(s_t, m_t \mid m_{1:t-1})$ is obtained as
\begin{equation}
    I(s_t,\hat m_t \mid \hat m_{1:t-1}) = I(s_t,\hat m_{1:t}) - I(s_t, \hat m_{1:t-1})\,.
\end{equation}
where $I(s_t, \hat m_{1:t-1})$ is the information that the receiver can infer about state $s_t$ before receiving message $\hat m_t$, while $I(s_t,\hat m_{1:t})$ is the mutual information between state $s_t$ and the entire sequence of messages $\hat m_{1:t}$. Therefore, $I(s_t, m_t \mid m_{1:t-1})$ is the conditional mutual information between $s_t$ and $\hat m_t$ given all past received messages, and represents the additional information about the state $s_t$ carried by the last message $\hat m_t$, which cannot exceed the channel capacity $C$
%This denotes how messages incrementally help reconstruct the state

This formulation clarifies the importance of designing a transmitter that keeps track not only of the current state of the system, but also of the information available to the receiver. On the other hand, the receiver must maintain a history of past messages, or a belief that is statistically equivalent to it, to limit redundancy between subsequent transmissions.

